PilotEar: Enabling In-ear Inertial Navigation

Navigation systems are used daily. While different types of navigation systems exist, inertial navigation systems (INS) have favorable properties for some wearables which, for battery and form factors may not be able to use GPS. Earables (aka ear-worn wearables) are living a momentum both as leisure devices, and sensing and computing platforms. The inherent high signal to noise ratio (SNR) of ear-collected inertial data, due to the vibration dumping of the musculoskeletal system; combined with the fact that people typically wear a pair of earables (one per ear) could offer significant accuracy when tracking head movements, leading to potential improvements for inertial navigation. Hence, in this work, we investigate and propose PilotEar, the first end-to-end earable-based inertial navigation system, achieving an average tracking drift of 0.15 m/s for one earable and 0.11 m/s for two earables.

==> sections/Acknowledgement.tex <==



